Subspace Robust Wasserstein Distances

Making sense of Wasserstein distances between discrete measures in high-dimensional settings remains a challenge. Recent work has advocated a two-step approach to improve robustness and facilitate the computation of optimal transport, using for instance projections on random real lines, or a preliminary quantization of the measures to reduce the size of their support. We propose in this work a "max-min" robust variant of the Wasserstein distance by considering the maximal possible distance that can be realized between two measures, assuming they can be projected orthogonally on a lower $k$-dimensional subspace. Alternatively, we show that the corresponding "min-max" OT problem has a tight convex relaxation which can be cast as that of finding an optimal transport plan with a low transportation cost, where the cost is alternatively defined as the sum of the $k$ largest eigenvalues of the second order moment matrix of the displacements (or matchings) corresponding to that plan (the usual OT definition only considers the trace of that matrix). We show that both quantities inherit several favorable properties from the OT geometry. We propose two algorithms to compute the latter formulation using entropic regularization, and illustrate the interest of this approach empirically.

==> sections/SRW2.tex <==
\section{The SRW$_2$ Distance}\label{sec:srw2}

Since orthogonal projections are fundamentally Euclidean, it is most natural to consider the case $p=2$. In this case, we prove that SRW$_2$ has a nice interpretation in terms of the eigendecomposition of the displacement second-order moment matrix $V_\pi$~\eqref{eq:vpi}: 
\begin{lemma} \label{lemma:dual_formulation}
For $k \in \range{d}$ and $\mu, \nu \in \PdRd$ one has that $\ProjWasserstein{k}^2(\mu, \nu)$ is equal to both values below:
\begin{align}
 \adjustlimits \min_{\pi \in \Pi(\mu,\nu)} \max_{E \in \G_k} \int \|P_E(x) - P_E(y)\|^2 d\pi(x,y) \label{eqn:maxmin} \\
\min_{\pi \in \Pi(\mu, \nu)} \sum_{l=1}^k \lambda_l(V_\pi) \label{eqn:minVpi}
\end{align}
\end{lemma}
\emph{Proof.} $\ProjWasserstein{k}^2(\mu, \nu)$ = \eqref{eqn:maxmin}:  
Let $W=\ProjWasserstein{k}^2$ and use Lemma~\ref{lemma:projected_transport_plans}
\[
	\begin{split}
		 W = \max_{E \in \G_k} \min_{\rho \in \Pi({P_E}_\#\mu , {P_E}_\#\nu)} \int \|x-y\|^2 \,d\rho(x,y) \\
= \max_{E \in \G_k} \min_{\pi \in \Pi(\mu, \nu)} \int \|P_E(x)-P_E(y)\|^2 \,d\pi(x,y).
	\end{split}
\]
We invert the minimum and the maximum.

\eqref{eqn:maxmin} = \eqref{eqn:minVpi} : We focus on the inner maximization in~\eqref{eqn:minVpi}. Using the variational formulation of the sum of the $k$ largest eigenvalues of a matrix,
\[
	 \sum_{l=1}^k \lambda_l(V_\pi) = \max_{\substack{U \in \R^{k \times d}\\UU^T = I_k}} \tr\left( U V_\pi U^T \right).
\]
Then plugging the definition of $V_\pi$ and taking the minimum over $\pi \in \Pi(\mu,\nu)$ yields \eqref{eqn:minVpi} = \eqref{eqn:maxmin}.\quad\quad$\square$



This characterization of SRW$_2$ as a sum of eigenvalues is crucial to study more precisely SRW$_2$ distances, and in particular to show that they can be computed as the maximum of a concave function over a convex set, which will make computations tractable.
\begin{theorem} \label{theo:convex_relaxation}
For $k \in \range{d}$ and $\mu, \nu \in \PdRd$,
\begin{align}
	\ProjWasserstein{k}^2(\mu, \nu) &= \min_{\pi \in \Pi(\mu, \nu)} \max_{\substack{0 \preceq \Omega \preceq I\\\tr(\Omega) = k}}  \int d_\Omega^2 \,d\pi \label{eqn:minmaxOmega} \\
	&= \max_{\substack{0 \preceq \Omega \preceq I\\\tr(\Omega) = k}} \min_{\pi \in \Pi(\mu, \nu)} \int d_\Omega^2 \,d\pi \label{eqn:maxOmegamin}
\end{align}
where $d_\Omega$ stands for the Mahalanobis distance
\[
	d_\Omega^2(x,y) = (x-y)^T \Omega (x-y).
\]
\end{theorem}
\emph{Proof}. $\ProjWasserstein{k}^2(\mu, \nu)$ = \eqref{eqn:minmaxOmega} : 
We fix $\pi \in \Pi(\mu, \nu)$ and focus on the inner maximization in~\eqref{eqn:minmaxOmega} :
\[
	\max_{\substack{0 \preceq \Omega \preceq I\\\tr(\Omega) = k}}  \int d_\Omega^2 \,d\pi = \max_{\substack{0 \preceq \Omega \preceq I\\\tr(\Omega) = k}}  \left\langle \Omega \,|\, V_\pi \right\rangle.
\]
A classical result by~\cite{fan1949theorem} shows that this is equal to
\[
	\max_{\substack{U \in \R^{k \times d}\\UU^T = I_k}}  \tr\left( U V_\pi U^T \right)
\]
which is nothing but the sum of the $k$ largest eigenvalues of $V_\pi$. Taking the minimum over $\pi \in \Pi(\mu, \nu)$ yields the result. To prove \eqref{eqn:minmaxOmega} = \eqref{eqn:maxOmegamin} we use Sion's minimax theorem to interchange the minimum and the maximum.$\quad\quad\square$

The following corollary of Theorem~\ref{theo:convex_relaxation}, for fixed $\pi \in \Pi(\mu,\nu)$, gives an optimal solution for the maximization:
\begin{corollary} \label{cor:optimalOmega_fixedpi}
For $\pi \in \Pi(\mu, \nu)$, compute the eigendecomposition of $V_\pi = U \diag\left( \lambda_1, ..., \lambda_d \right) U^T$
with $\lambda_1 \geq ... \geq \lambda_d$. Then for $k \in \range{d}$, $\widehat\Omega = U \diag\left([\ones_k, \zeros_{d-k}]\right) U^T$ solves
\[
	\max_{\substack{0 \preceq \Omega \preceq I\\\tr(\Omega) = k}}  \int d_\Omega^2 \,d\pi.
\]
\end{corollary}

